Made-to-measure galaxy models - II Elliptical and Lenticular Galaxies

We take a sample of 24 elliptical and lenticular galaxies previously analysed by the SAURON project using three-integral dynamical models created with Schwarzschild's method, and re-analyse them using the made-to-measure (M2M) method of dynamical modelling. We obtain good agreement between the two methods in determining the dynamical mass-to-light (M/L) ratios for the galaxies with over 80% of ratios differing by < 10% and over 95% differing by < 20%. We show that (M/L)_M2M is approximately equal to (M/L)_Sch. For the global velocity dispersion anisotropy parameter delta, we find similar values but with fewer of the made-to-measure models tangentially anisotropic by comparison with their SAURON Schwarzschild counterparts. Our investigation is the largest comparative application of the made-to-measure method to date.

==> abstract <==
We take a sample of 24 elliptical and lenticular galaxies previously analysed
by the SAURON project using three-integral dynamical models created with Schwarzschild's 
method, and re-analyse them using the made-to-measure (M2M) method of dynamical modelling.  
We obtain good agreement between the two methods in determining the dynamical mass-to-light 
(M/L) ratios for the galaxies with over 80% of ratios differing by < 10% and over 95% 
differing by < 20%. We show that (M/L)_M2M is approximately equal to (M/L)_Sch.   
For the global velocity dispersion anisotropy parameter \delta, we find similar values 
but with fewer of the made-to-measure models tangentially anisotropic by comparison with 
their SAURON Schwarzschild counterparts. Our investigation is the largest comparative 
application of the made-to-measure method to date.


